VideoGPA: Distilling Geometry Priors for 3D-Consistent Video Generation

While recent video diffusion models (VDMs) produce visually impressive results, they fundamentally struggle to maintain 3D structural consistency, often resulting in object deformation or spatial drift. We hypothesize that these failures arise because standard denoising objectives lack explicit incentives for geometric coherence. To address this, we introduce VideoGPA (Video Geometric Preference Alignment), a data-efficient self-supervised framework that leverages a geometry foundation model to automatically derive dense preference signals that guide VDMs via Direct Preference Optimization (DPO). This approach effectively steers the generative distribution toward inherent 3D consistency without requiring human annotations. VideoGPA significantly enhances temporal stability, geometric plausibility, and motion coherence using minimal preference pairs, consistently outperforming state-of-the-art baselines in extensive experiments.

==> sections/10-introduction.tex <==

\section{Introduction}
Recent video diffusion models\junjie{maybe add some references here} have achieved a milestone in visual fidelity and conditional flexibility. 
However, a fundamental gap remains: these models often \textit{lack a coherent understanding of 3D geometry under camera motion}.
Even state-of-the-art models frequently produce objects that deform unnaturally, drift spatially, or exhibit flickering occlusion boundaries when the viewpoint shifts.

We argue that this limitation does not primarily stem from insufficient model capacity. Modern video diffusion models are large and expressive, and many failure cases are visually close to valid solutions. Instead, we hypothesize that the issue arises from a \textit{misalignment between standard denoising objectives and geometric coherence}. While standard training encourages pixel-level realism, it does not explicitly reward the structural integrity required for a 3D-consistent world.

A key obstacle in addressing this problem is the lack of reliable and scalable diagnostics for geometric consistency. While prior work has explored explicit structural priors, such as point clouds~\cite{zhang2024worldconsistentvideodiffusionexplicit, hou2025trainingfreecameracontrolvideo} and 4D rendering~\cite{bai2025recammastercameracontrolledgenerativerendering}, to enforce consistency, these approaches often constrain the generative space and degrade performance in general video synthesis. Alternatively, geometry-based constraints derived from multi-view relations~\cite{zhang2024worldconsistentvideodiffusionexplicit, kupyn2025epipolar} tend to be sparse and noisy, making them difficult to integrate directly into diffusion training.

% We hypothesize that these failures arise not from a fundamental lack of architectural capacity, but from a misalignment between standard denoising objectives and geometric coherence.
% These artifacts reveal that current architectures lack an underlying stable 3D scene representation that persists across frames. 
% Crucially, a robust metric pipeline to diagnose and evaluate these geometric stability issues remains underdeveloped \cite{li2025videohalluevaluatingmitigatingmultimodal}. While many works have attempted to fix 3D consistency through explicit structural priors, such as point clouds \cite{zhang2024worldconsistentvideodiffusionexplicit, hou2025trainingfreecameracontrolvideo} or 4D rendering \cite{bai2025recammastercameracontrolledgenerativerendering}, these degrade video models' generative capabilities.
% Alternatively, multi-view geometry constraints~\cite{zhang2024worldconsistentvideodiffusionexplicit, kupyn2025epipolar} often provide noisy signals that are difficult to integrate directly into the latent space optimization of diffusion training.
% and those related to multi-view geometry (e.g., epipolar constraints \cite{zhang2024worldconsistentvideodiffusionexplicit, kupyn2025epipolar}). Nevertheless, these approaches face fundamental trade-offs and limitations. Methods that explicitly embed restrictive structural priors can limit the model’s generative capabilities, while traditional geometric losses are often noisy, susceptible to feature matching failures, and difficult to integrate directly into the latent space optimization inherent in diffusion training.

In parallel, recent progress in post-training alignment for diffusion models has demonstrated that large generative models can be steered effectively using preference-based optimization. A series of works adapt diffusion models to reinforcement learning or preference optimization frameworks by reformulating likelihood ratios in ODE- to SDE-based settings~\cite{wallace2023diffusionmodelalignmentusing, deng2024flowdpoimprovingllmmathematical, liu2025flowgrpotrainingflowmatching, xue2025dancegrpounleashinggrpovisual}. These methods suggest an immense potential for reshaping models’ output distribution through lightweight post-training.

% Recent breakthroughs in diffusion model fine-tuning have propelled this class of optimization methods into the spotlight. Post-training alignment frameworks have become central to effectively refining large generative models. This includes pioneering work that adapts $\text{ODE}$-based diffusion models to $\text{SDE}$-based $\text{RL}$ frameworks \cite{wallace2023diffusionmodelalignmentusing, deng2024flowdpoimprovingllmmathematical, liu2025flowgrpotrainingflowmatching, xue2025dancegrpounleashinggrpovisual}. These methods collectively demonstrate immense potential to steer model output toward desired qualities using preference signals. 

Motivated by this observation, we introduce \textbf{\methodname}, a post-training alignment approach for improving 3D geometric consistency in video diffusion models without introducing explicit structural priors or human annotations. As illustrated in Fig.~\ref{fig:Teaser}, \methodname applies a feed-forward geometric foundation model to generated videos to recover camera motion and scene structure, and uses the resulting reprojection consistency as a dense geometric signal. This signal serves as a preference objective to fine-tune video diffusion models via Direct Preference Optimization (DPO).

We show that with minimal post-training (LoRA fine-tuning on $\sim$1\% of model parameters), \methodname substantially improves geometric coherence under camera motion, while preserving the base model’s visual quality and motion realism. Across both image-to-video and text-to-video settings, \methodname consistently improves over prior art. These results suggest that geometric consistency in video diffusion models can be substantially improved through post-training objective alignment.

% \begin{itemize}
%     \item We bridge 3D reconstruction and video generation by incorporating geometric reconstruction models into the post-training optimization loop, enabling efficient geometry-aware refinement.
%     \item We introduce a geometry-guided alignment framework that distills a self-supervised 3D consistency signal into preference optimization, significantly improving geometric stability using only lightweight post-training updates and no human annotations or restrictive structural priors.
%     \item Through extensive experiments on image-to-video and text-to-video generation, we demonstrate that our approach effectively mitigates common 3D failure modes while preserving general-purpose video generation quality.
% \end{itemize}

% To address the limitations of existing geometric metrics and the high cost of human feedback~\cite{liu2025improvingvideogenerationhuman}, we introduce our \textbf{3D Consistency Score}. This score provides a \textbf{simple, reliable, fast, and dense geometric signal} derived from a 3D reconstruction pipeline under Occam's razor philosophy. We adopt VGGT-1B \cite{wang2025vggt} as our geometric backbone and design a fully GPU-accelerated pipeline, enabling the processing of dozens of frames in seconds. Furthermore, we ensure the entire process is differentiable for future research.

% In summary, our main contributions are:

% \textbf{Bridging 3D Reconstruction and Video Generation:} We propose a novel paradigm that incorporates 3D reconstruction models directly into the optimization loop of video diffusion models, transforming the video generation process from a pixel-interpolation task to a geometry-aware structural synthesis task.

% \textbf{Structural Alignment via Geometric Distillation:} We pioneer a geometry-guided optimization framework that aligns the latent space of CogVideoX with explicit 3D structural constraints. By distilling a 3D consistency signal into the fine-tuning loop, we effectively "rectify" the model’s motion manifold. This transformation resolves chronic pathological artifacts—such as structural collapse and temporal flickering—enabling the synthesis of high-fidelity videos that maintain rigid geometric integrity even under extreme, large-scale camera maneuvers.

% \textbf{3D Consistency Benchmark:} We establish a novel, autonomous benchmark derived from a robust 3D reconstruction pipeline. This serves as the first scalable metric to quantitatively evaluate both geometric structural coherence and camera motion diversity. Our benchmark provides a rigorous evaluation standard for the community, filling the void in metrics for 3D-consistent video synthesis.

% We construct a large dataset by applying our efficient 3D Consistency Score to a diverse set of generated videos. This dataset, annotated with our self-supervised geometric value signal, provides a valuable resource for future research in geometry-aware video generation and serves as a robust benchmark for model evaluation.


==> sections/60-limitation.tex <==
\section{Limitation}

\textcolor{blue}{We will add limitation and failure cases here}
